Analyzing Semantic Change through Lexical Replacements

Modern language models are capable of contextualizing words based on their surrounding context. However, this capability is often compromised due to semantic change that leads to words being used in new, unexpected contexts not encountered during pre-training. In this paper, we model \textit{semantic change} by studying the effect of unexpected contexts introduced by \textit{lexical replacements}. We propose a \textit{replacement schema} where a target word is substituted with lexical replacements of varying relatedness, thus simulating different kinds of semantic change. Furthermore, we leverage the replacement schema as a basis for a novel \textit{interpretable} model for semantic change. We are also the first to evaluate the use of LLaMa for semantic change detection.

==> Another_paper_based_on_TugofWords.tex <==
Firstly, we make a proof of concept by looking at the difference between the representation of all the context words and the target word. When the target is native in the context, then there is a much smaller distance between the representation of the target word and the average representation of the context words. When instead, we replace the target word with a synonym, this gap increases, and continues to increase as we replace more and more distantly related words. So, if a word r gains a completely novel senses (the sense of w), then the contextual models are not able to use the context words to replicate for r, the meaning of w. 

We study this displacement in three way: 
First the distance between the representation of the target word and the replacement word, next as the self-distance between the target word and the replacement word given the same context, and finally, in the WiC task where target words are replaced. 


Using the insights gained in this study, we develop a method for developing an interpretable approach to Lexical semantic change that outperforms current state of the art on the English portion of the SemEval-2020 Task 1 testset. 

==> main.tex <==
\section{Introduction}\label{sec:introduction}
The major novelty and advancement that contextualised BERT models have brought to language modelling is the ability to dynamically generate vector representations based on specific usage context: we can thus easily differentiate between \textit{sitting on a rock} and \textit{listening to rock}. 

%\begin{figure}[!ht]
%Francesco: if we place the figure here, we can ha ve it in page 1
%Francesco: Lave the sentence about AI models and BERT to motivate the use of DALL-E 2 as example.
%Francesco: I comment the figure as Luigi doesn't want it in the paper
%    \begin{center}
%        \includegraphics[width=0.37\columnwidth]{imgs/sit-at-meat.png}
%        \caption{Image generated by DALL-E 2 in response to the prompt \texttt{sit at a meat, cartoon}. This image exemplifies the limitations in contextualisation within AI models. We hypothesise similar \textit{misunderstandings} in BERT embeddings due to the excessive use of pre-trained knowledge.}
%        \label{fig:sit-at-meat}
%    \end{center}
%\end{figure}

While BERT models are \textit{pre-trained} on huge all-purpose corpora, typically with a large emphasis on web corpora, researchers and practitioners employ them for diverse text applications. Regardless of how well the information and language in the studied text align with the pre-training text, the models are used to generate word vector representations (i.e. embeddings) for any input sequence. However, this implies a gap between where the models have learned all of %(or, in case of fine-tuning, the majority of) 
their parameters, and the data on which they are applied. Indeed, BERT models serve as the lens through which we view the studied texts: if our texts are contemporary with the pre-training, the gap is likely to be minimal; if, however, we intend to study historical or other out-of-domain (OOD) corpora, this gap can be arbitrarily large and have major effects on follow-up studies. 

The effects can be exemplified in the area of Lexical Semantic Change (LSC) where the state of the art postulates a standard recipe: a word is modelled by its contextualised embeddings for different time periods~\cite{montanelli2023survey}. These representations are then compared over time to detect change. However, if BERT models impose too much pre-trained contemporary knowledge in a historical context, they are unable to generate accurate representations of the historical meaning of a word. For instance, the historical expression \textit{sit at meat} denotes taking a seat at the dining table or joining others for a meal\footnote{An example is the passage from the King James Bible (Luke 14:10): ``But when thou art bidden, go and sit down in the lowest room; that when he that bade thee cometh, he may say unto thee, Friend, go up higher: then shalt thou have worship in the presence of them that \textit{sit at meat} with thee.''}, as \textit{meat} originally referred to ``any kind of food''. Over time, the term underwent semantic narrowing and now typically refers to animal flesh used as food. Models relying heavily on contemporary pre-trained knowledge may not faithfully capture the authentic historical meaning of ``meat''. %, as illustrated in Figure~\ref{fig:sit-at-meat}. 
This could  result in an underestimation of semantic change. Similar effects may arise when studying language variation across speaker communities or in out-of-domain contexts, such as detecting hate speech~\cite{nozza2021exposing}, radicalization~\cite{sakketou2022investigating}, and dog whistles~\cite{denigot2020dogwhistles}. By studying the degree of influence that the model exerts versus the context, we can offset this in subsequent modelling, and build more contextualised models.

Some previous exploration of the contextualisation has been done, typically through probing tasks~\cite{jawahar2019bert}, or by analysing the geometry of the vector representations~\cite{ethayarajh2019contextual}. In this paper, we investigate to what degree the representation of a target word is determined by BERT's pre-trained knowledge and contra the context in which it appears by analysing the effect of substituting a \textit{target} word with a \textit{replacement} word and studying the impact on the corresponding contextualised  representations.\footnote{To reduce the amount of free variables, like spelling variations and OCR errors, in this study, we  focus on modern texts and will verify our findings on historical texts in future work.}

\paragraph{Our contributions:}

\begin{compactitem}
\item  Using a replacement schema, we analyse how the ``tug of war'' between the context and BERT's pre-trained knowledge affects the contextualisation. We find that the degree of BERT's contextualisation is not fixed but depends on the linguistic relations between the words, thereby reflecting the model's sensitivity to these linguistic features. We establish that contextualisation changes as a function of semantic relatedness which we systematically test across different linguistic relations, namely synonymy, antonymy, and hypernymy.    
\item We investigate BERT's contextualisation across different PoS classes and find that they are affected differently. We validate these findings through the Word-in-Context (WiC) task, revealing discrepancies between verbs and nouns. This implies that assessments for tasks like WiC should be tailored to different PoS to provide a more comprehensive evaluation, thereby enhancing the robustness of BERT models.
\item We challenge the use of BERT embeddings to capture semantic changes involving meanings beyond the pre-trained knowledge of BERT. We demonstrate that approaches relying on the clustering of BERT embeddings fall short in capturing semantic changes, as they struggle to correctly contextualise untuned word meanings.
\item  We propose a new interpretable approach to Lexical Semantic Change (LSC) by leveraging contextualised BERT embeddings. Our approach leverage lexical replacements and outperforms existing state-of-the-art (SOTA) achieving the top score for English. 
\end{compactitem}

\section{Related Work}\label{sec:related-work}
BERT-like models leverage the Transformer encoder to capture the semantics of words~\cite{devlin2019bert,vaswani2017attention}. Their success in solving NLP tasks has prompted numerous studies to explore the nature and characteristics of their contextualised architectures. \newcite{ethayarajh2019contextual,coenen2019visualizing,cai2021isotropy,jawahar2019bert} shed light on the geometry of the embedding space. \newcite{serrano2019attention,bai2021attentions,guan2020far} investigate the interpretability of the attention mechanism. \newcite{yenicelik2020bert,gari2021lets,kalinowski2021exploring,haber2021patterns} examine the clusterability of word representations. \newcite{abdou2022word,hessel2021effective,mickus2020mean,wang2021on} analyse the impact of word position in the embeddings generation. \newcite{coenen2019visualizing,levine2020sensebert,pedinotti2020dont} study how word meaning are represented in the embedding space. 

Most of the current work involves probing tasks, as proposed by~\citet{hewitt2019designing}. These tasks consist of training an auxiliary classifier on top of a model, where the contextualised embeddings serve as features to predict syntactic (e.g. PoS) and semantic (e.g. word relations) properties of words~\cite{clark2019bert,lin2022bert,Wallat2023probing,lin2022bert,ravichander2020systematicity}. If the auxiliary classifier accurately predicts a linguistic property, the property is assumed to be encoded in the model.  

Our work extends previous work that focus on the contextualisation of BERT-like models. Instead of using probing tasks, we leverage a replacement schema according to PoS and semantic categories with graded lexical relatedness. Like~\newcite{ethayarajh2019contextual,jawahar2019bert}, we analyse the contextualisation across all layers of BERT. Building on the work of~\newcite{zhao2020quantifying}, our research focuses on the degree of contextualisation. However, while they assess the inference of semantic word classes from contextualised embeddings, we analyze the contextualisation of different PoS that models exert under LSC and for OOD words. 

\section{Methodology}\label{sec:methodology}
In our experiments, we leverage a replacement schema to investigate the pre-trained contextualisation of BERT. This involves analyzing the variations in embedding representations when a target replacement is introduced.\footnote{Given our primary focus on words and their replacements when these words are split into multiple sub-words by the model, we calculate the average embeddings of the corresponding sub-words. This approach ensures the preservation of the same number of tokens in the original and artificial sentences and enables accurate distance calculations.} For instance, by replacing a target like \textit{cat} with a replacement like \textit{chair} in a specific context like \textit{The <target/replacement> was purring loudly}. 

\subsection{The replacement schema}\label{sec:replacement-schema}
We use WordNet to generate different classes of replacements for a specific word~\cite{Fellbaum1998}, which correspond to a varying degree of plausibility (i.e. suitability of a specific replacement) between the target word and its replacement. Thus, we hypothesise that each class is associated with a different impacts on contextualisation. Each class of replacements also has diachronic relevance, as the synchronic, semantic relation can be considered to have a parallel in semantic change~\cite{wegmann2020detecting}. To ensure accurate linguistic replacements, we maintain PoS agreement with the target words; that is, \textit{nouns} are replaced with \textit{nouns}, and so forth. %Examples are given in the form (target $\leftarrow$ replacement) in Table~\ref{tab:lex-repl}. %remove comment in CAMERA READY

\begin{compactitem}
\item \texttt{synonyms} (e.g. \textit{sadness}~$\leftarrow$~\textit{unhappiness}) are used to evaluate the stability in contextualisation; that is, we hypothesise similar embeddings between target and replacement words. Indeed, synonyms are considered equally likely alternatives in BERT's pre-trained knowledge. On the diachronic level, they emulate the absence of any semantic change of the replacement word;

\item \texttt{antonyms} (e.g. \textit{hot}~$\leftarrow$~\textit{cold}) are used to evaluate a light change in contextualisation; that is, we hypothesise slightly less similar embeddings between target and replacement words. Indeed, antonyms are sometimes equally plausible alternatives\footnote{For example: I \textit{love/hate} you} while other times are likely to surprise the model\footnote{For example: I burned my tongue because the coffee was too \textit{hot/cold}}. On the diachronic level, they emulate the a contronym change\footnote{A contronym change occurs when a word's new meaning is the opposite of its original meaning (e.g. \textit{sanction} in English)} of the replacement word;

\item \texttt{hypernyms} (e.g. \textit{bird}~$\leftarrow$~\textit{animal}) are used similarly to \texttt{antonyms}. However, on the diachronic level, they emulate a broadening semantic change of the replacement word;

\item \texttt{random} words (e.g. \textit{sadness}$~\leftarrow$~\textit{eld}) are used to evaluate a change in contextualisation. If BERT places high importance on the context, then the replacement should receive a similar representation to the target word. Otherwise, if BERT heavily relies on its pre-trained knowledge, the replacement will exhibit dissimilarity to the target word despite the identical context, as well as dissimilarity to the typical replacement representations. On the diachronic level, \texttt{random} emulates the presence of strong semantic change of the replacement word, that is the emergence of a homonymic sense.

\item \texttt{synthetic} words (e.g. \textit{love} $\leftarrow$ \textit{new-token}) are used as a baseline to evaluate the contextualisation of word meanings regardless of pre-trained knowledge. Indeed, we add a new token in the BERT's pre-trained vocabulary, and as such, it does not have any associated pre-trained knowledge (i.e., untuned weights). We hypothesise very dissimilar embeddings between target and synthetic words. On the diachronic level, this class mimics the adaptation to newly emerging concepts beyond their specific training time frame or to new domains. 
\end{compactitem}

\begin{comment}%remove comment in CAMERA READY
\begin{small}
\begin{table*}[!ht]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{llllllllll}
\textbf{Lexical Replacement} & 
\multicolumn{1}{c}{\textbf{$w^{-4}$}} & 
\multicolumn{1}{c}{\textbf{$w^{-3}$}} & 
\multicolumn{1}{c}{\textbf{$w^{-2}$}} & 
\multicolumn{1}{c}{\textbf{$w^{-1}$}} & 
\multicolumn{1}{c}{\textbf{$w \ / \ w^{(r)}$}} & 
\multicolumn{1}{c}{\textbf{$w^{+1}$}} & 
\multicolumn{1}{c}{\textbf{$w^{+2}$}} & 
\multicolumn{1}{c}{\textbf{$w^{+3}$}} & 
\multicolumn{1}{c}{\textbf{$w^{+4}$}} \\
Target Word                                            & moments                                                         & of                                                              & regret                                                 & and                                                    & \textit{sadness}                                                & and                                                    & guilty                                                 & relief                                                 & .                                                      \\
Synonym                                                & moments                                                         & of                                                              & regret                                                 & and                                                    & \textit{unhappiness}                                            & and                                                    & guilty                                                 & relief                                                 & .                                                      \\
Hypernym                                               & moments                                                         & of                                                              & regret                                                 & and                                                    & \textit{feeling}                                                & and                                                    & guilty                                                 & relief                                                 & .                                                      \\
Antonym                                                & moments                                                         & of                                                              & regret                                                 & and                                                    & \textit{happiness}                                              & and                                                    & guilty                                                 & relief                                                 & .                                                      \\
Random                                                 & moments                                                         & of                                                              & regret                                                 & and                                                    & \textit{eld}                                                    & and                                                    & guilty                                                 & relief                                                 & .                                                     
\end{tabular}%
}
\caption{Different classes of replacements.}
\label{tab:lex-repl}
\end{table*}
\end{small}
\end{comment}

\subsection{Data}\label{sec:data}
To avoid introducing noise into our experiments resulting from the conflation of senses, we replace words with contextually appropriate replacements based on the intended sense of the word within a specific sentence (e.g, \textit{stone} and \textit{music} for \textit{sitting on a rock} and \textit{listening to rock}, respectively). We therefore leverage the SemCor dataset~\cite{MillerLTB93}, still the largest and most commonly used sense-annotated corpus for English. To select candidate replacements,  we consider different PoS tags, namely \textit{verbs}, \textit{nouns}, \textit{adjectives} and \textit{adverbs}, and semantic classes, namely \textit{synonyms}, \textit{hypernyms} and \textit{antonyms}. We randomly sample a set of synsets for each PoS tag occurring in SemCor, and for a specific synset, we extract a subset of sentences where a word is annotated with that synset. We sample a maximum of 10 sentences per synset to prevent oversampling of high-frequency synsets. For each sentence, we generate the \textit{synonym} and  \textit{antonym} replacements for all PoS, and \textit{hypernym} replacements only for nouns and verbs\footnote{WordNet lacks hypernym information for other PoS} (see  Table~\ref{tab:semcor_stats}). 

%PIERLUIGI: why are there very few adverb compared to other PoS?
\begin{table}[!ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|r|r|r|}
\hline
\textbf{PoS} & \multicolumn{1}{l|}{\textbf{N. target words}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Avg. sampled senteces\\ per target word\end{tabular}}} & \multicolumn{1}{l|}{\textbf{N. examples}} \\ \hline
noun         & 360                                           & 3.55                                                                                                          & 1277                                      \\ \hline
verb         & 433                                           & 3.45                                                                                                          & 1494                                      \\ \hline
adjective    & 393                                           & 3.39                                                                                                          & 1334                                      \\ \hline
adverb       & 158                                           & 3.46                                                                                                          & 546                                       \\ \hline
\end{tabular}%
}
\caption{Data statistics over  PoS, sampled from SemCor.}
\label{tab:semcor_stats}
\end{table}


\subsection{Tug of War in BERT}
We delve into the intricate dynamics of the tug of war that occurs within the contextualisation of words by focusing on the word contextualisation (Section~\ref{sec:contextualisation}), and the use of replacements as a proxy for semantic change (Section~\ref{sec:lexical-semantic-change}). In our experiments, we utilise word embeddings generated by the monolingual BERT base model\footnote{\textit{bert-base-uncased}} due to its widespread usage. Additional analyses for XLM-R\footnote{\textit{xlm-roberta-base}} and mBERT\footnote{\textit{bert-base-multilingual-cased}} are presented in appendix\footnote{\textbf{All code, experimental results, and data will be released under a public license upon acceptance.}}. 

\section{Word contextualisation}\label{sec:contextualisation}
We analyse the word contextualisation by comparing the embeddings of a word $w$ in the original sentence to those in the same sentence when $w$ is replaced by $r$. To perform this comparison, we rely on the cosine distance between the embeddings of $w$ and $r$. We refer to this distance as the \textit{self-embedding distance} (SED), i.e.,

\begin{center}
\resizebox{0.8\columnwidth}{!}{%
$\begin{matrix}\label{mat:self-emb-dist}
w^{-n}  & ... & w^{-1} & w & w^{+1}  & ... & w^{+m}\\ 
 &   & \ & \updownarrow &   &   & \\
w^{-n}  & ... & w^{-1} & r & w^{+1}  & ... & w^{+m}\\
\end{matrix}
$
}
\end{center}
\noindent \newline
where $w^{-n}, ..., w^{-1}$ and $w^{+1}, ..., w^{+m}$  denotes the embeddings of $n$ and $m$ neighbouring words to the left and right of the target word $w$, respectively.\footnote{Given our primary focus on words and their replacements when these words are split into multiple sub-words by the model, we calculate the average embeddings of the corresponding sub-words. This approach ensures the preservation of the same number of tokens in the original and synthetic sentences and enables accurate distance calculations.}
The higher the SED, the less BERT leverages context to contextualise words but instead relies on pre-trained knowledge. 

\subsection{Self-embedding distance}
\label{sec:sedsection}
For each pair of original and artificial sentences, we computed SED across each layer. We then analysed the average SED for each class of replacement and PoS at each BERT layer. To address the anisotropic nature of BERT's space\footnote{Embeddings occupy a narrow cone within the vector space~\cite{ethayarajh2019contextual}.} and ensure comparability across layers, we normalise the average SED score for each class of replacements with the average SED score obtained with \texttt{synthetic} replacements. We report average SED scores in Figure~\ref{fig:self-embedding-distance}.

 \begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{imgs/self-embedding-distance.png}
    \caption{Average SED over layers.}
    \label{fig:self-embedding-distance}
\end{figure*}


Like~\newcite{ethayarajh2019contextual}, we observe that the word contextualisation increases across layers as the SED decreases. However, we find a similar degree of contextualisation in the last layers of BERT, indeed the SED becomes somewhat stable for each class of replacements and PoS. Adverbs represents an exceptional case, as the word contextualisation is less stable than other class of replacements. 

For \texttt{adverb}, the \texttt{synonyms} and \texttt{antonyms} are closer than for other PoS, while being, along with \texttt{random}, associated with lower SED; that is, adverbs are more contextualised than other PoS and less pre-trained knowledge is used for their representation. This is most likely because adverbs in English are more context-dependent than the other PoS. Indeed, they can modify verbs, adjectives, adverbs, and entire sentences, in contrast to adjectives, which may only modify nouns and pronouns, and to verbs and nouns, which constitute essential components of sentences. This finding is in line with the work of~\newcite{lorge2023wacky}, which shows \textit{weak differentiation amongst the semantic classes of adverbs}. 

For other PoS, the SED score for \texttt{random} is above 1.0 in all layers, leading us to argue that BERT falls short in contextualising out-of-context words when pre-trained knowledge is available. That is, the representation of a random word does not mimic the representation of the target word that it replaces. The context thus has minimal effect in determining the representation of the replacement word. 

For \texttt{verb}, we note a higher SED for \texttt{antonyms, synonyms}, and \texttt{hypernyms} in comparison to other PoS. Additionally, there is a narrower gap between the SED for \texttt{random} and the SED for \texttt{antonyms, synonyms, hypernyms}. These observations suggest that the contextualisation of verbs is less pronounced than that of other PoS and that the model relies more on pre-trained knowledge. As a result, the embeddings of verbs exhibit greater similarity to the embeddings of random words in context.

As for \texttt{adjective} and \texttt{noun}, we note that they exhibit similar contextualisation across layers. Additionally, for \texttt{noun}, \texttt{hypernyms} are less similar to the target than \texttt{antonyms} and \texttt{synonyms}. This aligns with the recent findings of~\newcite{hanna2021analyzing}, suggesting that BERT's understanding of noun hypernyms is limited.  

All in all, our results suggest that models exhibit varying degrees of contextualisation for different PoS, with lower contextualisation observed for verbs.


\subsection{PoS contextualisation through WiC} 
To verify that the variations in contextualisation across PoS are not an artifact of the replacement schema, we utilise Word-in-Context (WiC),  a popular task in NLP for which various benchmarks are available in different languages. WiC is a recent task designed to assess the effectiveness of contextualised embeddings in capturing word usages by determining whether a target word $w$, occurring in a pair of sentences $\langle s1, s2\rangle$, has the same meaning or not~\cite{pilehvar2019wic}. 

PoS information is available for most WiC benchmarks but, thus far, existing approaches to WiC have treated all PoS as a bundle. For our experiments, we consider benchmarks for different languages: English (WiC-en~\citealp{pilehvar2019wic}, MCL-WiC-~\citealp{martelli2021semeval}), French (MCL-WiC-fr~\citealp{martelli2021semeval}), Italian (XL-WiC-it~\citealp{raganato2020xl}, WiC-ITA-it~\citealp{evalita2023wicita}), and German (DWUG-de~\citealp{schlechtweg2020semeval})\footnote{Although the benchmark for French and German provided by~\newcite{raganato2020xl} is considerably larger, we have made the decision not to use them due to the presence of noisy instances that could potentially impact our analysis negatively.}. We split the WiC benchmarks into distinct sub-corpora for nouns, verbs, and adjectives\footnote{We excluded adverbs due to the limited number of examples.}. Details on the benchmarks are available in Appendix~\ref{app:wic}. 

Following~\newcite{pilehvar2019wic}, we tune a threshold-based classifier on the development set (Dev) of each WiC benchmark, PoS, and BERT layer, totaling 216 classifiers\footnote{6 benchmarks, 3 PoS, 12 layers}. For each sentence pair available in a Dev set, we computed the cosine similarity between the contextualised embeddings of the target word $w$ extracted individually from a layer of a BERT model\footnote{We use \textit{bert-base-uncased} for English, \textit{dbmdz/bert-base-french-europeana-cased} for French, \textit{dbmdz/bert-base-french-italian-uncased} for Italian, \textit{bert-german-cased} for German. The models are base versions of BERT with 12 attention layers and a hidden layer of size 768.}. The threshold for a classifier is determined by optimising the F1-score over Dev and then applied to both the Train and Test sets. Instead of using accuracy as an evaluation metric, we employ the F1-score to account for the inherent class imbalance in these split benchmarks.


\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
 &
  \multicolumn{2}{c}{\textbf{WiC-en}} &
  \multicolumn{2}{c}{\textbf{MCL-WiC-en}} &
  \multicolumn{2}{c}{\textbf{XL-WiC-fr}} &
  \multicolumn{2}{c}{\textbf{XL-WiC-it}} &
  \multicolumn{2}{c}{\textbf{WiC-ITA-it}} &
  \multicolumn{2}{c}{\textbf{DWUG-de}} \\ \cline{2-13} 
\multicolumn{1}{c|}{} &
  \textit{Train} &
  \multicolumn{1}{c|}{\textit{Test}} &
  \textit{Train} &
  \multicolumn{1}{c|}{\textit{Test}} &
  \textit{Train} &
  \multicolumn{1}{c|}{\textit{Test}} &
  \textit{Train} &
  \multicolumn{1}{c|}{\textit{Test}} &
  \textit{Train} &
  \multicolumn{1}{c|}{\textit{Test}} &
  \textit{Train} &
  \multicolumn{1}{c|}{\textit{Test}} \\ \cline{2-13} 
\multicolumn{1}{c|}{\textit{nouns}} &
  \textbf{0.691} &
  \multicolumn{1}{c|}{\textbf{0.683}} &
  \textbf{0.796} &
  \multicolumn{1}{c|}{\textbf{0.847}} &
  \textbf{-} &
  \multicolumn{1}{c|}{\textbf{0.677}} &
  \textbf{0.678} &
  \multicolumn{1}{c|}{\textbf{0.689}} &
  0.682 &
  \multicolumn{1}{c|}{\textbf{0.759}} &
  \textbf{0.808} &
  \multicolumn{1}{c|}{\textbf{0.799}} \\
\multicolumn{1}{c|}{\textit{verbs}} &
  0.615 &
  \multicolumn{1}{c|}{0.611} &
  0.752 &
  \multicolumn{1}{c|}{0.805} &
  \textbf{-} &
  \multicolumn{1}{c|}{0.622} &
  0.639 &
  \multicolumn{1}{c|}{0.593} &
  0.459 &
  \multicolumn{1}{c|}{0.615} &
  0.630 &
  \multicolumn{1}{c|}{0.640} \\
\multicolumn{1}{c|}{\textit{adjectives}} &
  \textbf{-} &
  \multicolumn{1}{c|}{\textbf{-}} &
  0.738 &
  \multicolumn{1}{c|}{0.819} &
  - &
  \multicolumn{1}{c|}{0.653} &
  \textbf{-} &
  \multicolumn{1}{c|}{\textbf{-}} &
  \textbf{0.733} &
  \multicolumn{1}{c|}{0.695} &
  \textbf{-} &
  \multicolumn{1}{c|}{\textbf{-}} \\ \cline{2-13} 
  %
  \multicolumn{1}{c|}{\textit{Acc.}} &
  \multicolumn{2}{c|}{{0.638}} &

  \multicolumn{2}{c|}{0.840} &
  \multicolumn{2}{c|}{0.787} 
 &
  \multicolumn{2}{c|}{{0.726}} &
  \multicolumn{2}{c|}{Macro-F1 0.670} &
  \multicolumn{2}{c|}{{-}} \\ 
    %
  \multicolumn{1}{c|}{\textit{Reference}} &
  \multicolumn{2}{c|}{\citeauthor{pilehvar2019wic}} &
  \multicolumn{2}{c|}{\citeauthor{martelli2021semeval}} &
  \multicolumn{2}{c|}{\citeauthor{martelli2021semeval}} 
 &
  \multicolumn{2}{c|}{\citeauthor{raganato2020xl} } &
  \multicolumn{2}{c|}{\citeauthor{periti2023time}} &
  \multicolumn{2}{c|}{{}} \\ 
  \cline{2-13} 
\end{tabular}%
}
\caption{Scores obtained by threshold-based classifiers for WiC trained on Dev sets. Results are provided for PoS and WiC benchmarks, with the best result in each considered benchmark and dataset highlighted in \textbf{bold}. The bottom rows show the SOTA accuracy and corresponding reference reported for the benchmark.}
\label{tab:wic-roc}
\end{table*}

For the sake of brevity, we report in Table~\ref{tab:wic-roc} results for classifiers based on last layer embeddings. Additional and consistent results for each layers are reported in Appendix~\ref{app:wic}. According with the finding of Figure~\ref{fig:self-embedding-distance}, we find that BERT consistently performs better at distinguishing usages of nouns than verbs, with adjectives falling in between. 

As \textit{verbs are approximately twice as polysemous as nouns}~\cite{lin2001structure}, we want to exclude that WiC performance over PoS is not influenced varying levels of polysemy instead of the models' contextualisation capability. We analysed the polysemy distributions of target words for each PoS and benchmark, finding that a comparable degree of polysemy for each PoS in the considered WiC benchmarks. This assessment involved checking the polysemy of each target word in the various WiC benchmarks using Open Multilingual Wordnet, for English, French, Italian~\cite{Fellbaum1998}, and Odenet for German~\cite{siegel2021odenet}.  See Appendix \ref{app:polysemy} for details. These results lead us to conclude that BERT exhibits varying degree of contextualisation for different PoS.


\section{Semantic change}\label{sec:lexical-semantic-change}
Lexical Semantic Change (LSC) is the task of automatically identifying words that change their meaning over two (or more) time-specific corpora $C_1$ and $C_2$~\cite{tahmasebi2021survey,tahmasebi2023computational,montanelli2023survey}.
Recently, there has been growing attention towards this task, fuelled by shared competitions and benchmarks such as  \citet{schlechtweg2020semeval,basile2020diacr, kutuzov2021rushifteval}.  % like SemEval-2020 Task 1~\cite{schlechtweg2020semeval}, DIACR-Ita~\cite{basile2020diacr}, RuShiftEval-21~\cite{kutuzov2021rushifteval}, and LSCDiscovery-22~\cite{zamora2022lscdiscovery}.
With the advent of contextualised language models, these competitions act as additional benchmarks to assess the capability of contextualised embeddings in capturing word meanings. The current benchmarks consist of diachronic corpora $C_1$ and $C_2$ and a reference set of target words annotated with a degree of semantic change between $C_1$ and $C_2$. The goal is to rank the target words according to their degree of lexical semantic change.

\subsection{Form-based and sense-based approaches}\label{app:form-sense}
Approaches to LSC relying on contextualised word embeddings are typically distinguished into two main categories: \textit{form-based} approaches and \textit{sense-based} approaches~\cite{montanelli2023survey}. The former captures semantic change by solely relying on similarities among raw embeddings without depending on sense disambiguation and representation. A common strategy involves aggregating all the embeddings of a word in $C_1$ and $C_2$ by averaging, and modeling the change as the cosine similarity of the average representations (PRT)~\cite{martinc2020leveraging}
. The latter generally use clustering algorithm like Affinity Propagation to identify senses and subsequently model the change as divergence of cluster distributions (JSD)~\cite{martinc2020capturing}. %Francesco: the two works are different

We argue that our findings in Section~\ref{sec:contextualisation} has important implications on these approaches when pre-trained models are used. Specifically, consider semantic changes involving the acquisition or loss of new/old meanings. When these semantic changes occurs, if BERT models lack pre-trained knowledge of the involved meanings, they tend to position the corresponding word embeddings instances far apart in the space from the other embeddings of the same word, regardless of the context in which the word occurs (see \texttt{random} in Fig~\ref{fig:self-embedding-distance}). While \textit{form-based} approaches may still detect semantic changes by identifying low-contextualised word occurrences, \textit{sense-based} approaches fall short in accurately detecting the same semantic changes. This is because they require modelling meanings outside the model's pre-trained knowledge before detecting those changes. Since these meanings cannot be adequately modeled, given the model's low degree of contextualisation, the performance of \textit{sense-based} approaches is reduced compared to that of \textit{form-based} approaches.
%: 1) \textit{form-based} can accurately recognise semantic changes by identifying low-contextualised word occurrences (see \texttt{random} in Fig~\ref{fig:self-embedding-distance}) that the model tends to position far in the space from other embeddings of the same word; 2) conversely, \textit{sense-based} approaches fall short in accurately recognising semantic changes as they require modelling meanings outside the model pre-trained knowledge as clusters of similar word embeddings. However, these clusters cannot be properly modeled, as the embeddings for new meanings outside the pre-trained knowledge suffer from a low degree of contextualisation. This implies that the semantic change cannot be recognised by the emergence of a new cluster, thus reducing performance on LSC.

We further tested these implications in the LSC task by comparing PRT and JSD on an artificial diachronic corpus spanning two time periods (see details in Appendix~\ref{app:synthetic-LSC}). Essentially, we introduced random replacements in $C_2$ with varying probabilities to emulate different degrees of change for a set of 46 target words. Subsequently, we compared the Spearman Correlation between the scores obtained with PRT and JSD with the artificially graded score of emulated semantic change. Results using BERT are presented in Figure~\ref{fig:random-LSC} (see Appendix~\ref{app:synthetic-LSC} for additional results). Our hypothesis is that while PRT can accurately predict changes, JSD falls short because it can only correctly model the meanings that BERT is already aware of.

As shown in the figure, we can accurately model artificial semantic changes, even from layer 2, using PRT. This is not the case for JSD, where we observe statistically significant correlations for only a few layers. However, the significance of performance for JSD is an artifact of BERT embeddings and does not authentically represent the simulated change. We verify this by examining the modelled clusters. While, in general, the number of clusters of AP is large~\cite{martinc2020capturing,periti2022done}, representing \textit{sense nodules}\footnote{Lumps of meaning with greater stability under contextual changes~\cite{Cruse2000-CRUAOT-2}} rather than word meanings~\cite{kutuzov2022contextualized}, we find that the injected confusion in the model due to the \texttt{random} replacements results in a very low number of clusters (typically 2, maximum of 4). We report similar results in Appendix for other languages (i.e. German, Swedish, Spanish)%TODO

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{imgs/random-LSC.png}
    \caption{Spearman Correlation over layers for artificial semantic change.}
    \label{fig:random-LSC}
\end{figure}


\subsection{Addressing LSC through replacements}
As a further contribution of this paper, we propose a novel supervised\footnote{According to the classification framework presented by~\citet{montanelli2023survey}} approach to Graded Change Detection building upon the replacement schema. Our approach leverages a curated set of word replacements from WordNet and Wiktionary. 

We denote  $T=\{w_1,w_2,...,w_N\}$ as the set of target words. For each target word, we extract a set of possible replacements $\rho(w_i) = \{r_1,r_2,...,r_M\}$, resulting in $N*M$ replacement pairs. The set of replacements is obtained by considering the lemmas of synonyms and hypernyms associated with the target word $w_i$ in WordNet and words extracted from the Wiktionary page corresponding to the target word. For each target word $w_i$, we sample up to 200 sentences from each period that remain stable regardless of the replacement word $r_j$. %, i.e. $S_{t_1}$ and  $S_{t_2}$. %Then, we create as far synthatic sub-corpora S_t_1 and S_t_2 as the number of considered replacements.
For each replacement pair ($w_i,r_j$), we denote the set of sentences  for a time period $t\in\{1,2\}$ as $S^t(w_i,r_j)$.%\footnote{The set of sentences in $S^t(w_i,r_j)$ are fixed for each target word $w_i$, only the replacement word $r_j$ changes.} 


%%%%%%%%%%%%%5555
For each sentence $s\in S^t(w_i,r_j)$ we measure the self-embedding distance of the target and replacement word and denote it $sed(s)$. 
%the average sentence distance is $awd (s) = \frac{1}{n+m}\sum_{i=-n}^{ m}d^i$, where $d^i$ is the self-embedding distance of the i-th word in $s$ (Section \ref{sec:repldist}). 
%%%%%%%%%%%%%%%%
%
The average self-embedding distance of a target-replacement pair is defined as \[awd^t(w_i,r_j) = \frac{1}{|S^t(w_i,r_j)|}\sum_{s \in S^t(w_i,r_j)} sed(s)\]


The absolute difference in $awd$ over time is denoted 
TD$(w_i,r_j)$. % = \left | \text{awd}^2(w_i,r_j) - \text{awd}^1(w_i,r_j) \right | \]
Finally, we rank the replacements $\rho(w_i)$ according to their degree of time difference:
\begin{small}
\[R(\rho(w_i)) = \{r_1,r_2,...,r_M | \ \text{TD}(w_i,r_{i+1},)\leq \text{TD}(w_i,r_{i})\}\]
\end{small}
and we compute a semantic change score $lsc_{w}$ as the average TD considering the top $k$ replacements: 
\[lsc_w = \frac{1}{k}\sum_{r \in R(\rho(w_i))_k} \text{TD}(w_i,r)\] %where $R(\rho(w))_k = {v_1,v_2,...,v_k}$.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{imgs/spearman2.png}
    \caption{Top-k replacement vs Spearman Correlation.}
    \label{fig:spearman-top-k-replacement}
\end{figure}

We evaluate our approach on the SemEval-2020 Task 1, Subtask 2 dataset for English. We compute the Spearman Correlation between the graded score reported in the gold truth and the $lsc$ scores. Figure~\ref{fig:spearman-top-k-replacement} reports the correlation computed for different values of $k$. The highest correlation of 0.741 is achieved when considering the first 22 replacements, while the lowest correlation of 0.600 is obtained using only the first replacement (see Table~\ref{tab:eng_lsc_results}). Interestingly, the minimum correlation obtained using the replacements is competitive with SOTA results. Moreover, on average, the correlation is higher than the SOTA model's performance. The replacements are reported in Table \ref{ref:eng_changes}. We used the linguistically-aware replacement strategy in the LSC task to assess and quantify the semantic changes undergone by words over time. By replacing the target words with different semantically related words, we generate contextual variations that enable the detection of semantic shifts. In the case of words like \textit{record} and \textit{land} that have undergone semantic change through narrowing and generalisation, respectively, linguistically aware replacement scan provide valuable insights.  The replacement process generates a list of replacements that can be used as labels for the types of semantic change observed. By associating each replacement with a specific semantic category or change type, it becomes possible to analyse and quantify the semantic shifts experienced by words over time.

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
 & \textbf{Model} & \textbf{Spearman Correlation} \\ \cline{2-3} 
 & \citeauthor{rosin2022temporal} & 0.629 \\
 & \citeauthor{kutuzov2020uio} & 0.605 \\
 &  \citeauthor{laicher} & 0.571 \\
 &  \citeauthor{periti2022done} & 0.512 \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Synonym \\ Replacement\end{tabular}}} & Replacement Min. Corr. & 0.600 \\
 & Replacement Max. Corr. & 0.741 \\
 & Replacement Avg. Corr. & 0.674 \\
 \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Random \\ Replacement\end{tabular}}} & Replacement Min. Corr. & 0.495 \\
 & Replacement Max. Corr. & 0.622 \\
 & Replacement Avg. Corr. & 0.542
\end{tabular}%
}
\caption{Spearman Correlation on SemEval-2020 Task 1 (Eng), where our results outperform current SoTA.}
\label{tab:eng_lsc_results}
\end{table}

\subsection{Random replacements}
In this section, we present results using randomly selected words with the same Part of Speech (PoS) as the target word, i.e. \texttt{random} replacement as introduced in Section~\ref{sec:methodology}. This approach generates a list of substitute words contextually unrelated to the target word. Some interesting patterns emerge when these results are compared with those obtained using synonym replacement. In the case of semantic change detection, the use of synonyms can provide more contextually relevant replacements, as they share semantic relationships with the target word. However, using random word replacements can still yield reasonable results, as evidenced by an average correlation of 0.542. These results is in line with the finding of Section~\ref{app:form-sense}.

In these approach, although random replacements tend to perform worse than synonym replacements, they have one distinct advantage: they do not rely on external lexical resources. This way, the approach is also suitable for unsupervised scenarios. While synonym replacements can improve contextualisation and semantic relevance, they are not always readily available or reliable for languages with limited linguistic resources. In such cases, random word replacements can still provide reasonable results and serve as a practical and resource-efficient approach for tasks where synonym information is scarce or unavailable.

In Section \ref{sec:sedsection}, by using SemCor, we effectively account for the nuances of different word senses, thereby improving the contextualisation and semantic relevance of synonym replacements. This approach is more targeted as synonyms are selected based on their association with a particular sense, leading to higher quality contextualisation in the context of that sense. As a result, synonym replacements are more finely tuned to the specific meaning of the target word, reducing noise and improving correlation with semantic change labels.

The lower correlations observed with random replacements indicate that contextualisation effects vary significantly when unrelated words are introduced into the context. This emphasizes the crucial role of context in the performance of language models when they have prior knowledge of input word meanings. However, it should not be assumed that contextualisation is equally effective when modeling new meanings outside the scope of the model's pre-trained knowledge.

\section{Conclusions}

Ethayarajh’s work~\citeyearpar{ethayarajh2019contextual}, which was the first to study  contextualisation in a methodical way,
has clearly set the stage for our fine-grained study of  contextualisation. We extend this line of work by studying the ``tug of war'' between BERT's contextualisation and its pre-trained knowledge respect to the area of LSC and OOD.

In this paper, we analyse the degree of contextualisation using a replacement schema that can be used for any pre-trained LLMs. We focus on BERT and find that contextualisation effects differ across PoS. We support this finding by splitting up WiC datasets and find that the results are consistently better for nouns than verbs, across several languages, an effect that cannot be attributed to polysemy effects. We also conclude that the pre-training models significantly influence the representation of a word, and BERT models are not capable of capturing contextualised word meanings beyond their pre-training. Thus, our results indicate that the low degree of contextualisation can have severe limiting effects when pre-trained BERT models are applied  to out-of-domain text. We will further verify these findings using, for example, historical, sense-tagged texts. 

Using the same replacement schema, we demonstrate that \textit{form-based} approaches are more suitable than \textit{sense-based} approaches for detecting semantic changes when pre-trained models are employed. Additionally, we propose a novel approach to LSC and are able to surpass the results achieved by existing state-of-the-art models in the task of LSC. Our replacement schema gives us an automatic way of providing labels for the change that has occurred, offering us a way to do explainable semantic change detection. In future work, we will use models that utilise the complete encoder-decoder architecture, such as T5~\cite{raffel2020exploring}, or exclusively the decoder architecture such as GPT-like models~\cite{brownlanguage2020}, to  generate replacement categories without relying on existing resources like WordNet. We will also evaluate the degree of contextualisation on these models. 

\section*{Limitations}
One potential limitation of our study lies in the use of the replacement schema in conjunction with lexical replacements generated from WordNet. As a matter of fact, inherent limitations of WordNet, such as potential gaps, inaccuracies, or ambiguities in the semantic relationships may influence our analysis. WordNet also limits the data sources from which we can draw sentences, since we need a corpus with sense annotations corresponding to a lexicon. 

Furthermore, in our experiment, the lexical replacement process involves substituting a \textit{word} occurrence in the original sentence with a related \textit{lemma} extracted from WordNet. As a result, providing the model with synthetic sentences containing the lemma instead of the inflected word may influence the generation of word embeddings and the contextualisation of every word in the sentences. However, we assume that this limitation equally affects every class we consider. For example, while the lemma of a verb may reduce the third singular verb form, the plural forms of adjectives and nouns can also be simplified to singular lemma forms. Additionally, to mitigate these issues and ensure that all PoS are equally affected by the replacement procedure, we replaced both the target and replacement words with lemmas in the original and synthetic sentences, respectively.

Finding the correct form of a replacement requires advanced morphological analysis and carries the risk of leading to errors. For now, we therefore opted to circumvent this by replacing targets and lemmas alike. Furthermore, we would like to highlight a relevant study by~\newcite{laicher} that delves into the influence of various linguistic variables on the use of BERT embeddings for the LSC task. This research demonstrates that by reducing the influence of orthography through lemma usage, significant enhancements in BERT's performance were observed for German and Swedish, while maintaining comparable results for English. This underscores the potential benefits of lemma-based contextualisation and that linguistic features like orthography can sometimes be minimised without substantial loss of performance.



==> old.tex <==
%Our experiments show that this pull is directly related to the linguistic relationship (such as hyponomy or antonomy) between the original word and its replacement, and thus, the relationship between the replacement (i.e., the semantically changing word) and its novel context.}

%Francesco: I don't think we need the sentence below
%Similar effects may arise when studying language variation across speaker communities or in OOD contexts, such as detecting hate speech~\cite{nozza2021exposing}, radicalization~\cite{sakketou2022investigating}, and dog whistles~\cite{denigot2020dogwhistles}. %By studying the degree of influence that the model exerts versus the context, we can offset this in subsequent modeling, and build more contextualized models.


%~\cite{su2022improving,rosin2022time} introduced novel temporal objectives for Masked Language Models (LMLM) aimed at enhancing the models' ability to generalize temporally and contextualize word representations. Similarly,~\cite{rosin2022temporal} extended the attention mechanism underlying these models to facilitate the generation of time-specific embeddings. 

%Our work extends previous work that focus on the contextualization of BERT-like models. Instead of using probing tasks, we leverage a replacement schema according to PoS and semantic categories with graded lexical relatedness. Like~\newcite{ethayarajh2019contextual,jawahar2019bert}, we analyze the contextualization across all layers of BERT. Building on the work of~\newcite{zhao2020quantifying}, our research focuses on the degree of contextualization. However, while they assess the inference of semantic word classes from contextualized embeddings, we analyze the contextualization of different PoS that models exert under LSC and for OOD words. 

